Summary of the searches for squarks and gluinos using $\sqrt{s}$ = 8 TeV pp collisions with the ATLAS experiment at the LHC

A summary is presented of ATLAS searches for gluinos and first- and second-generation squarks in final states containing jets and missing transverse momentum, with or without leptons or b-jets, in the $\sqrt{s}$ = 8 TeV data set collected at the Large Hadron Collider in 2012. This paper reports the results of new interpretations and statistical combinations of previously published analyses, as well as a new analysis. Since no significant excess of events over the Standard Model expectation is observed, the data are used to set limits in a variety of models. In all the considered simplified models that assume R-parity conservation, the limit on the gluino mass exceeds 1150 GeV at 95% confidence level, for an LSP mass smaller than 100 GeV. Furthermore, exclusion limits are set for left-handed squarks in a phenomenological MSSM model, a minimal Supergravity/Constrained MSSM model, R-parity-violation scenarios, a minimal gauge-mediated supersymmetry breaking model, a natural gauge mediation model, a non-universal Higgs mass model with gaugino mediation and a minimal model of universal extra dimensions.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 23-Mar-2015

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC,
Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP,
Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC,
China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic;
DNRF, DNSRC and Lundbeck Foundation, Denmark; EPLANET, ERC and NSRF, European Union;
IN2P3-CNRS, CEA-DSM/IRFU, France; GNSF, Georgia; BMBF, DFG, HGF, MPG and AvH
Foundation, Germany; GSRT and NSRF, Greece; RGC, Hong Kong SAR, China; ISF, MINERVA, GIF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO, Netherlands; BRF and RCN, Norway; MNiSW and NCN, Poland; GRICES and FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MSTD,
Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa;
MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SER, SNSF and Cantons of
Bern and Geneva, Switzerland; NSC, Taiwan; TAEK, Turkey; STFC, the Royal
Society and Leverhulme Trust, United Kingdom; DOE and NSF, United States of
America.

The crucial computing support from all WLCG partners is acknowledged
gratefully, in particular from CERN and the ATLAS Tier-1 facilities at
TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France),
KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain),
ASGC (Taiwan), RAL (UK) and BNL (USA) and in the Tier-2 facilities
worldwide.
%----------------------------------------------

==> inclsqgl_symmarypaper-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{Summary of the searches for squarks and gluinos using $\sqrt{s} = 8 \TeV$ $pp$ collisions with the ATLAS experiment at the LHC}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% Authors and list of contributors to the analysis
% \AtlasAuthorContribute also adds the name to the author list
% Include package latex/atlascontribute to use this
% Use authblk package if there are multiple authors, which is included by latex/atlascontribute
% \usepackage{authblk}
% \renewcommand\Authands{, } % avoid ``. and'' for last author
% \renewcommand\Affilfont{\itshape\small} % affiliation formatting
% \AtlasAuthorContributor{First AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasAuthorContributor{Second AtlasAuthorContributor}{b}{Author's contribution.}
% \AtlasAuthorContributor{Third AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasContributor{Fourth AtlasContributor}{Contribution to the analysis.}
% \author[a]{First Author}
% \author[a]{Second Author}
% \author[b]{Third Author}
% \affil[a]{One Institution}
% \affil[b]{Another Institution}

% If a special author list should be indicated via a link use the following code:
% Include the two lines below if you do not use atlasstyle:
% \usepackage[marginal,hang]{footmisc}
% \setlength{\footnotemargin}{0.5em}
% Use the following lines in all cases:
% \usepackage{authblk}
% \author{The ATLAS Collaboration%
% \thanks{The full author list can be found at:\newline
%   \url{https://atlas.web.cern.ch/Atlas/PUBNOTES/ATL-PHYS-PUB-2014-007/authorlist.pdf}}
% }

% Date: if not given, uses current date
%\date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{2.6}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{SUSY-2014-06}

\PreprintIdNumber{CERN-PH-EP-2015-162}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2014-XXX}
% \AtlasNote{ATL-PHYS-PUB-2014-XXX}
% \AtlasNote{ATL-COM-PHYS-2014-XXX}

% arXiv identifier
% \arXivId{14XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
% \AtlasJournal{Phys.\ Lett.\ B.}
% \AtlasJournalRef{\PLB 789 (2014) 123}
% \AtlasDOI{}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{A summary is presented of ATLAS searches for gluinos
and first- and second-generation squarks in final states containing jets and missing transverse momentum, with or without leptons or $b$-jets, in the $\sqrt{s}$ = 8 TeV data set collected at the Large Hadron Collider in 2012. This paper reports the results of new interpretations and statistical combinations of previously published analyses, as well as a new analysis. 
Since no significant excess of events over the Standard Model expectation is observed, the data are used to set limits in a variety of models.  
In all the considered simplified models that assume R-parity
conservation, the limit on the gluino mass exceeds 1150 GeV at 95\%
confidence level, for an LSP mass smaller than 100 GeV. Furthermore, exclusion limits are set for left-handed squarks in a phenomenological MSSM model, a minimal Supergravity/Constrained MSSM model, R-parity-violation scenarios, a minimal gauge-mediated supersymmetry breaking model, a natural gauge mediation model, a non-universal Higgs mass model with gaugino mediation and a minimal model of universal extra dimensions.}
%In simplified models considered, gluino masses up to 1330 GeV and squark masses up to 850 GeV are excluded
%In the mSUGRA/CMSSM model %with $\tan\beta = 30$, $A_0 = -2m_0$ and $\mu>0$ 
%gluino masses smaller than 1280 GeV are excluded. In the mGMSB model, a limit on the SUSY breaking scale $\Lambda$ up to 90 TeV is set.  


%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% List of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{0L-razor}{https://cds.cern.ch/record/1752911}
\AtlasCoverSupportingNote{1L+7jets}{https://cds.cern.ch/record/1751602}
\AtlasCoverSupportingNote{0L+1L combination}{https://cds.cern.ch/record/1754430}
\AtlasCoverSupportingNote{0L pMSSM onestep qL}{https://cds.cern.ch/record/1749919}
\AtlasCoverSupportingNote{SS/3L 5-body Gtt extension}{https://cds.cern.ch/record/1966089}
\AtlasCoverSupportingNote{Two-step grid with taus reinterpretation}{https://cds.cern.ch/record/1747021}
\AtlasCoverSupportingNote{0L reintepretation (appendix O, N)}{http://cds.cern.ch/record/1595965}
\AtlasCoverSupportingNote{Monojet reinterpretation}{https://cds.cern.ch/record/1744984}

% \AtlasCoverSupportingNote{Short title note 2}{https://cds.cern.ch/record/YYYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{29 June 2015}

% Analysis team members -- Indicate the Contact Editors (usually two) by (*) after their name
\AtlasCoverAnalysisTeam{Jean-Francois Arguin~(*), Geert-Jan Besjes,
Philip Bechtle,                       
Daniel Bullock, Roger Caminal, Sascha Caron, Arely Cortes-Gonzalez,
Orjan Dale, 
Ingrid Deigaard, Otilia Ducu, Amir Farbin, William Fawcett, Cora Fischer, Thomas Gillam, Vincent Giangiobbe, Louise Heelan, Gregor Herten~(*), Naoko Kanaya, Alex Kastanas, Evgeniy Khramov, Alex Koutsman, Anton
Kravchenko, Wolfgang Liebig, Anna Lipniacka, Jeanette
Lorenz, Nikola Makovec, Zach Marshall, Bertrand Martin dit Latour,
Mario Martinez-Perez, Antoine Marzin, 
Julien Maurer, Ljiljana Morvaj, Brian Petersen, Milind Purohit, Oliver
Ricken, Zuzana
Rurikova, Fabrizio Salvatore, Steffen Schaepe, Martin Johannes
Schultens, Valentina Tudorache, Pedro Urrejola, Marija Vranjes Milosavljevic~(*), Da Xu}

% Editorial Board Members --- Indicate the Chair by a (*) after his/her name
% Give either all members at once (then they appear on one line), or separately
\AtlasCoverEdBoardMember{Carl Gwilliam ~(*), Donatella Cavalli, Jean-Francois Grivaz, Marcel Vos}
% \AtlasCoverEdBoardMember{EdBoard~Chair~(*)}
% \AtlasCoverEdBoardMember{EB~Member~1}
% \AtlasCoverEdBoardMember{EB~Member~2}
% \AtlasCoverEdBoardMember{EB~Member~3}

% A PUB note has readers and not an EdBoard -- give their names here (one line or several entries)
% \AtlasCoverReaderMember{Reader~1, Reader~2}
% \AtlasCoverReaderMember{Reader~1}
% \AtlasCoverEdBoardMember{Reader~2}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-susy-2014-06-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-susy-2014-06-editorial-board@cern.ch}


